Machine Learning Techniques for Data Reduction of Climate Applications

Scientists conduct large-scale simulations to compute derived quantities-of-interest (QoI) from primary data. Often, QoI are linked to specific features, regions, or time intervals, such that data can be adaptively reduced without compromising the integrity of QoI. For many spatiotemporal applications, these QoI are binary in nature and represent presence or absence of a physical phenomenon. We present a pipelined compression approach that first uses neural-network-based techniques to derive regions where QoI are highly likely to be present. Then, we employ a Guaranteed Autoencoder (GAE) to compress data with differential error bounds. GAE uses QoI information to apply low-error compression to only these regions. This results in overall high compression ratios while still achieving downstream goals of simulation or data collections. Experimental results are presented for climate data generated from the E3SM Simulation model for downstream quantities such as tropical cyclone and atmospheric river detection and tracking. These results show that our approach is superior to comparable methods in the literature.

==> problem.tex <==

%E3SM is an extensively coupled Earth system and climate model that is utilized in mission-defined endeavors within the U.S. Department of Energy as well as various international model inter-comparison efforts~\cite{golaz2019doe}. Our experiments utilize the atmospheric data obtained from E3SM's high-resolution (HR) configuration coupled simulation. The atmospheric grids are constructed using a topology known as cubed-sphere. The HR grid configuration is characterized by 120 quadrilateral spectral elements in both $x$ and $y$ directions of each face of the cubed sphere corresponding to an approximate grid spacing of \SI{25}{\kilo\meter} and a total of 800,000 columns per variable per snapshot. 

In this work, we use the atmospheric field data simulated by E3SM and TempestExtreme Version 2.1 [] for TC tracking and AR detection. TempestExtreme is a software package specialized in feature tracking and scientific analysis for global Earth-system data. TempestExtremes tracks tropical cyclones through a two-step process. Firstly, it identifies potential nodes of tropical cyclones in each time interval by assessing the combination of lower sea-level pressure and the presence of a well-defined warm core in the upper atmosphere associated with nearby low-pressure systems. Following this initial step, numerous candidate TC nodes are identified and saved. Secondly, the system uses a series of criteria to determine which trajectories are excluded. These criteria include restrictions on the maximum distance of travel, the minimum duration of the life cycle, and the maximum allowable gap between consecutive nodes on a trajectory. This process effectively separates and connects qualified individuals, allowing for the creation of paths that extend across multiple time periods. As a result, a set of hurricane locations is generated, each defined by their latitude and longitude coordinates, and connected by a unique trajectory ID. For the above algorithm, five variables are used as inputs: pressure at sea-level (PSL), temperature at 500 hPa and 200 hPa (T500, T200), and zonal and meridional wind speed at surface (UBOT, VBOT).

For atmospheric river (AR) detection, TempestExtremes employs a comparable approach. Within each time slice, possible AR structures are identified by applying a threshold to the Laplacian of the integrated vapor transport field (IVT) and considering a minimum connected area. After that, the eligible candidate regions are connected to create trajectories while maintaining the requirement for a minimum fractional area overlap between consecutive time steps. The position of atmospheric rivers (AR) is represented using a set of binary masks, each of which matches the resolution of the input data. 

%






